Motion Planning in Irreducible Path Spaces

The motion of a mechanical system can be defined as a path through its configuration space. Computing such a path has a computational complexity scaling exponentially with the dimensionality of the configuration space. We propose to reduce the dimensionality of the configuration space by introducing the irreducible path --- a path having a minimal swept volume. The paper consists of three parts: In part I, we define the space of all irreducible paths and show that planning a path in the irreducible path space preserves completeness of any motion planning algorithm. In part II, we construct an approximation to the irreducible path space of a serial kinematic chain under certain assumptions. In part III, we conduct motion planning using the irreducible path space for a mechanical snake in a turbine environment, for a mechanical octopus with eight arms in a pipe system and for the sideways motion of a humanoid robot moving through a room with doors and through a hole in a wall. We demonstrate that the concept of an irreducible path can be applied to any motion planning algorithm taking curvature constraints into account.

==> images/cspace.tex <==
\usetikzlibrary{arrows}
\pgfarrowsdeclarecombine{twotriang}{twotriang}%
{triangle 90}{triangle 90}{triangle 90}{triangle 90}
\begin{figure}[h!]
\centering
\begin{tikzpicture}

        \newcommand{\uangle}{\mathbin{\rotatebox[origin=c]{90}{$\rrangle$}}}

        \draw[-,line width = 0.8pt] (0,0) -- (4,0) node[pos=0.5,below,fill=white] {$q_1$};
        \draw[-,line width = 0.8pt] (0,0) -- (0,4) node[pos=0.5,left,fill=white] {$q_2$};

        %\draw[-,line width = 0.8pt] (0,0) -- (0,4) node[pos=0.5,left,fill=white] {$q_2$}; \draw[-,line width = 0.8pt] (0,4) -- (4,4) node[pos=0.5,above] {$\uangle$}; 
        %\draw[-,line width = 0.8pt] (4,0) -- (4,4)
        %node[pos=0.5,right]{$\rrangle$};

         \path (4,0) edge[->-,thick] (4,4);
         \path (0,0) edge[->>-,thick] (4,0);
         \path (0,0) edge[->-,thick] (0,4);
         \path (0,4) edge[->>-,thick] (4,4);

        \draw [black,line width=0.8pt,fill=black!20] plot [smooth cycle]
                coordinates {(0.2,0.2) (1,2) (2,2) (1.8,0.8)};
        \draw [black,line width=0.8pt,fill=black!5,opacity=0.4,text opacity=1] plot [smooth cycle] coordinates
                {(1,1) (1,3.5) (3,3) (3,1) (2,0.5)};
        \draw [black,line width=0.8pt] plot [smooth cycle] coordinates
                {(1,1) (1,3.5) (3,3) (3,1) (2,0.5)};
        \node[above] at (1.5,3) {$\C_{FM}$};
        \node[above] at (1.7,1.5) {$Q$};

        \coordinate (p) at (0.7,0.5);
        \draw[color=black,fill=black] (p) circle (2pt) node[left]{$p$};
        \draw[color=black,fill=black,->,line width=0.8pt] (p) -- (1.07,0.85);

\end{tikzpicture}

\caption{Schema of a Configuration Space $\C$, with Constraint Manifold $\C_{FM} \subset
\C$, and the irreducible manifold $Q$. A random sample $p \in Q$ is projected
onto $Q \cap \C_{FM}$ to make it physically feasible.
\label{constraint_manifold_and_irreducible_set}}

\end{figure}


==> src/authors.tex <==
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/authors/Andreas_Orthey.png}

Andreas Orthey is JSPS Postdoctoral Fellow at the AIST Institution in Tsukuba, Japan. He obtained his M.Sc.
degree in 2012 from the Technical University of Berlin, Germany, and his Ph.D.
in 2015 from the INPT in Toulouse, France.  His research interests are
high-dimensional motion planning, humanoid robotics and artificial intelligence.

\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/authors/Olivier_Roussel.png}

Olivier Roussel obtained his M.S. degree in Robotics from University of Toulouse III in 2010.
He worked as a Research Engineer at CEA-List from April 2010 to June 2012 on
humanoid path planning and crowd simulation. In 2015, he obtained his Ph.D. at
LAAS-CNRS and University of Toulouse III under the supervision of Dr. Michel
Taïx as part of the ANR Flecto project in collaboration with CEA-List and
KineoCAM.

\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/authors/Olivier_Stasse.jpg}

Olivier Stasse is senior CNRS research scientist at LAAS-CNRS, Toulouse. He was
assistant professor in Computer Science at University of Paris 13. In 2000, he
received a Ph.D. in Intelligent Systems from University of Paris 6 under the
supervision of P. Coiffet, and the French Habilitation to Direct Research (HDR)
in Robotics (2013) from University of Toulouse III. His research interests are
mostly focused on humanoid robotics, and more specifically motion generation
motivated by vision. From 2003 to 2011, he was part of the funding members of
the Joint French-Japanese Robotics Laboratory (JRL) in Tsukuba, Japan created
by P. Coiffet and K.Tanie.

\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/authors/Michel_Taix.png}

Michel Ta\"ix is an Associate Professor in Control and Robotics at Université de Toulouse,
southern France. He teaches at the Université Paul Sabatier, and conducts his
research at LAAS-CNRS, in the GEPETTO group. His research interests include
motion planning, interactive planning, planning for humanoid robots and planning
for compliant and deformable objects (ANR Flecto project). 

